Large Language Models for Intent-Driven Session Recommendations

Intent-aware session recommendation (ISR) is pivotal in discerning user intents within sessions for precise predictions. Traditional approaches, however, face limitations due to their presumption of a uniform number of intents across all sessions. This assumption overlooks the dynamic nature of user sessions, where the number and type of intentions can significantly vary. In addition, these methods typically operate in latent spaces, thus hinder the model's transparency.Addressing these challenges, we introduce a novel ISR approach, utilizing the advanced reasoning capabilities of large language models (LLMs). First, this approach begins by generating an initial prompt that guides LLMs to predict the next item in a session, based on the varied intents manifested in user sessions. Then, to refine this process, we introduce an innovative prompt optimization mechanism that iteratively self-reflects and adjusts prompts. Furthermore, our prompt selection module, built upon the LLMs' broad adaptability, swiftly selects the most optimized prompts across diverse domains. This new paradigm empowers LLMs to discern diverse user intents at a semantic level, leading to more accurate and interpretable session recommendations. Our extensive experiments on three real-world datasets demonstrate the effectiveness of our method, marking a significant advancement in ISR systems.

==> plot/bad-case.tex <==
\begin{table}[t]
\small
\caption{The number and ratio of bad cases on test sets.}\label{tab:bad-case}
\addtolength{\tabcolsep}{-3pt}
\vspace{-0.15in}
\centering
\begin{tabular}{ccc|ccc|ccc}
\toprule
\multicolumn{3}{c|}{Opt-ML-1M}
&\multicolumn{3}{c|}{Opt-Games}
&\multicolumn{3}{c}{Opt-Bundle} \\\hline
ML-1M  &Game &Bundle &ML-1M  &Game &Bundle &ML-1M  &Game &Bundle \\\midrule 
3 &83 &18 
&1 &68 &23 
&3 &60 &26\\ 
0.30\% &8.30\% &7.56\%
&0.10\% &6.80\% &9.66\%
&0.30\% &6.00\%&10.92\%\\
\bottomrule
\end{tabular}
\end{table}


% \begin{table}[t]
% \small
% \caption{The number of bad cases on all datasets.}\label{tab:bad-case}
% \addtolength{\tabcolsep}{2pt}
% \vspace{-0.15in}
% \centering
% \begin{tabular}{c|cccc}
% \toprule
% &ML-1M  &Games &Bundle  \\\midrule
% \# Tested Sessions &1000 &1000 &238\\ 
% \# Bad Cases &3 &68 &25\\
% Ratio &0.30\% &6.80\% &10.50\%\\
% \bottomrule
% \end{tabular}
% \end{table}


==> plot/parameter.tex <==
\begin{table}[t]
\footnotesize
\addtolength{\tabcolsep}{-2pt}
\centering
\caption{The best parameter settings for baselines.}
\label{tab:parameter}
\vspace{-0.15in}
\begin{tabular}{c|c|c|cccc}
\toprule
& Parameter &Search Space &ML &CD &Ga. &Bu.\\\midrule
\rotatebox[origin=c]{90}{SKNN} &$K$ &$[50,100,150]$ &&&& \\\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{FPMC}} &$d$ &$[32,64,128]$ &&&& \\
&lr &$[10^{-4},10^{-3},10^{-2}]$&&&&\\
&batch\_size &$[64,128,256]$ &&&&\\\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{NARM}} &$d$ &$[32,64,128]$&&&& \\
&lr &$[10^{-4},10^{-3},10^{-2}]$&&&&\\
&batch\_size &$[64,128,256]$ &&&&\\
&hidden\_size &$[50, 100, 150, 200]$ &&&&\\
&layers &$[1,2,3]$ &&&&\\
\hline
STAMP &&&&&& \\
GCE-GNN &&&&&& \\
MCPRN &&&&&& \\
HIDE &&&&&& \\
Atten-Mixer &&&&&& \\
\bottomrule
\end{tabular}
\end{table}

==> section/conclusion-v2.tex <==
\section{Conclusion}
Inspired by the reasoning capability of LLMs, we introduce a new paradigm -- PO4ISR -- for intent-aware session recommendation. It aims to discover varying numbers of semantic intents hidden in different sessions for more accurate and comprehensible recommendations through iterative prompt optimization. Specifically, the Prompt Initialization module first creates the initial prompt to instruct LLMs to predict the next item by inferring varying intents reflected in a session. Then, the prompt optimization module is devised to optimize prompts with iterative self-reflection in an automatic manner. Finally, the prompt selection module seeks to appropriately select optimal prompts based on the robust generalizability of LLMs across diverse domains.  
Extensive experiments on real-world datasets show the superiority of PO4ISR against other counterparts. Furthermore, several insightful discoveries are made to guide subsequent studies in this area. 


% Inspired by the reasoning capability of LLMs, we introduce a new paradigm -- PO4ISR -- for intent-aware session recommendation. It aims to discover varying numbers of semantic intents hidden in different sessions for more accurate and comprehensible recommendations through iterative prompt optimization. PO4ISR mainly consists of three modules, including prompt initialization (PromptInit), Prompt Optimization (PromptOpt), and Prompt Selection (PromptSel). In particular, PromptInit creates the initial prompt to instruct LLMs to predict the next item by inferring varying intents reflected in a session. Then, PromptOpt is devised to optimize prompts with iterative self-reflection in an automatic manner. Finally, PromptSel seeks to appropriately select optimal prompts based on the robust generalizability of LLMs across diverse domains.  
% Extensive experiments on three real-world datasets demonstrate the superiority of PO4ISR against other counterparts. Furthermore, several insightful discoveries are made to guide subsequent studies in this area. 


==> section/conclusion.tex <==
\section{Conclusion}
Inspired by the advanced logical reasoning capability of LLMs, this paper introduces a new paradigm -- PO4ISR -- for intent-aware session recommendation. It aims to discover dynamic number of semantic intents hidden in different sessions for more accurate recommendation through iterative prompt optimization. PO4ISR mainly consists of three modules, including prompt initialization (PromptInit), Prompt Optimization (PromptOpt) and Prompt Curation (PromptCura).
PromptInit creates the initial prompt to instruct LLMs to predict the next item by inferring potential intents reflected in a session. Then, PromptOpt is devised to optimize prompts with self-reflection in an automatic manner. Finally, PromptCura seeks to appropriately select optimal prompt based on the cross-domain performance.  
Extensive experiments on three real-world datasets demonstrate the superiority of PO4ISR against other counterparts. Furthermore, several insightful discoveries are made with the goal of providing guidance for subsequent studies. 


==> section/experiment-v2.tex <==
\section{Experiments and Results}


\input{plot/comparison}

We conduct extensive experiments to answer five research questions\footnote{Our code and data are available at \url{https://github.com/llm4sr/PO4ISR}}. (\textbf{RQ1}) Does PO4ISR outperform baselines? (\textbf{RQ2}) How do different components affect PO4ISR? (\textbf{RQ3}) How do essential parameters affect PO4ISR? (\textbf{RQ4}) How does PO4ISR provide comprehensible SR? (\textbf{RQ5}) Is there any limitation of PO4ISR?

\subsection{Experimental Setup}
\subsubsection{Datasets}
We use three real-world datasets from various domains. In particular, MovieLen-1M (ML-1M)\footnote{\url{https://grouplens.org/datasets/movielens/}} contains users' ratings of movies. Games is one subcategory from the Amazon dataset~\cite{ni2019justifying}, containing users' ratings towards various video games. Bundle~\cite{sun2022revisiting} contains session data for three subcategories (Electronic, Clothing, and Food) of Amazon, where the intents for each session are explicitly annotated via crowdsourcing workers. Table~\ref{tab:statistics} shows the statistics of the datasets. For ML-1M and Games, we chronologically order the rated items into a sequence for each user and then divide it into sessions by day. For each dataset, we split the sessions into training, validation, and test sets with a ratio of 8:1:1, i.e., 80\% of the initial sessions are treated as training sets; the subsequent 10\% as the validation set; and the final 10\% as the test set.  

\subsubsection{Baselines} We compare our proposed PO4ISR with ten baselines, which can be classified into three types. \textit{The first type is the conventional methods}. \textbf{Mostpop} recommends the most popular items; \textbf{SKNN}~\cite{jannach2017recurrent} recommends session-level similar items; and
\textbf{FPMC}~\cite{rendle2010factorizing} is the matrix factorization method with the first-order Markov chain.
%
\textit{The second type is the deep learning-based methods, which can be categorized into single-intent and multi-intent based ones}.
\textbf{NARM}~\cite{li2017neural} is an RNN-based model with the attention mechanism to capture the main purpose from the hidden states;
\textbf{STAMP}~\cite{liu2018stamp} learns the general intention of users by emphasizing the effect of the last item in the context;
\textbf{GCN-GNN}~\cite{wang2020global} uses both local and global graphs to learn item representation thus obtaining the main intent of the session; 
\textbf{MCPRN}~\cite{wang2019modeling} models users’ multiple purposes to get the final session representation; 
\textbf{HIDE}~\cite{li2022enhancing} splits the item embedding into multiple chunks, with each chunk representing a specific intention to learn diverse intentions within context;
and \textbf{Atten-Mixer}~\cite{zhang2023efficiently}: learns multi-granularity consecutive user intents to generate more accurate session representations.
%
\textit{The last type is the LLM-based method}.
\textbf{NIR}~\cite{wang2023zero} adopts zero-shot prompting for the next item recommendation.


\subsubsection{Parameter Settings}
We use Optuna (\url{optuna.org}) to automatically find out the optimal hyperparameters of all methods with 50 trails. In particular, the maximum training epoch is set as 100 with the early stop mechanism. 
The search space for batch size, item embedding size,
and learning rate are 
$\{64,128,256\}, \{32,64,128\}$ and $\{10^{-4},10^{-3},10^{-2}\}$, respectively.    
For SKNN, $K$ is searched from $\{50,100,150\}$. 
For NARM, the hidden size and layers are searched in $[50, 200]$ stepped by 50 and in $\{1,2,3\}$, respectively.
For GCE-GNN, the number of hops, and the dropout rate for global and local aggregators are respectively searched in $\{1,2\}, [0, 0.8]$ stepped by 0.2, and $\{0, 0.5\}$.  
For MCPRN, $\tau$ and the number of purpose channels are separately searched in $\{0.01, 0.1, 1, 10\}$ and $\{1,2,3,4\}$.
For HIDE, the number of factors is searched in $\{1,3,5,7,9\}$; the regularization and balance weights are searched in $\{10^{-5},10^{-4},10^{-3},10^{-2}\}$; the window size is searched in $[1,10]$ stepped by 1; and the sparsity coefficient is set as 0.4.
For Atten-Mixer, the intent level $L$ and the number of attention heads are respectively searched in $[1,10]$ stepped by 1 and in $\{1,2,4,8\}$.
For PO4ISR, $N=50, N_t=32, N_r=2, N_o=4, E_1=16, E_2=2$; and we randomly select 8 prompts as the input of the UCB Bandits in each iteration.  

\subsubsection{Evaluation Metrics}
Following state-of-the-arts~\cite{yin2023understanding,wang2019modeling,wang2023zero}, HR@K and NDCG@K are adopted as the evaluation metrics. We set $K=1/5$ since most users tend to prioritize the quality of items appearing at the top positions in real scenarios~\cite{liu2021top}. Generally, higher metric values indicate better ranking results. 
For a fair comparison, the candidate size of all methods is set as 20 following NIR~\cite{wang2023zero};
all non-LLM baselines are trained with 150 randomly sampled sessions from the training set, while PO4ISR uses the subset of 50 sessions. This is because although PO4ISR uses 50 sessions to optimize prompts in each domain, it considers the performance from (three) diverse domains for the final prompt selection. For non-LLM baselines, it is non-trivial to use the cross-domain performance to select the best models. This also helps showcase the superior advantages of LLMs on generalization.  
%
To manage the API call cost, for ML-1M and Games, we randomly sample 1000 sessions from the validation set and test set, respectively. 
For robust performance, we repeat the test procedure five times where each time we set different seed values (e.g., 0, 10, 42, 625, and 2023) to generate different candidate sets. Finally,  we report the average results as presented in Table~\ref{tab:comparison}.  

\input{plot/ablation}
\input{plot/cross-domain-test}


\subsection{Results and Analysis}

\subsubsection{Overall Comparison (RQ1)}

Table~\ref{tab:comparison} shows the performance of all methods on the three datasets. Several findings are noted. 

\textbf{(1)} Regarding conventional methods (CMs), the model-based FPMC performs the best on sparser datasets Games and Bundles, while is slightly defeated by SKNN on the denser dataset ML-1M (see `Density Indicator' in Table~\ref{tab:statistics}). This exhibits the strong capability of model-based methods in learning sequential patterns with sparse data. \textbf{(2)} For single-intent methods (SIMs), each gains its best performance on different datasets, e.g., NARM excels on ML-1M, whereas GCE-GNN wins on Games. Generally, GCE-GNN showcases advantages on shorter sessions with sparser datasets (e.g., Games). This is because such sessions do not contain sufficient local information, thus requiring global information (graph) to compensate. Conversely, NARM performs well on longer sessions with denser datasets (e.g., ML-1M), since such sessions possess substantial information (e.g., frequent patterns) making the fusion of global information potentially noisy. \textbf{(3)} Concerning multi-intent methods (MIMs), MCPRN displays the poorest performance across all datasets, as limited training data hinders the learning of proper parameters for multiple RNN channels. Besides, HIDE exceeds Atten-Mixer on relatively denser datasets (ML-1M and Games) but lags on the sparsest Bundle.
\textbf{(4)} Among LLM-based methods (LLMMs), PO4ISR outperforms NIR, corroborating our prior assertion that basic in-context learning fails to fully exploit LLMs, thereby emphasizing the superiority of our prompt optimization paradigm.  

Overall, CMs underperform SIMs or MIMs, underscoring the importance of capturing user intents for improved SR. The victory of MIMs over SIMs on Bundle validates the effectiveness of multi-intent learning. However, some of the SIMs (e.g., NARM) surpass MIMs (e.g., MCPRN) on ML-1M and Games, suggesting that fixed numbers of intents might constrain the capability of MIMs. LLMMs exhibit strength on sparser datasets compared to denser ones (e.g., NIR on Games vs. ML-1M), and shorter sessions compared to longer ones (e.g., NIR on Games vs. Bundles). Similar trends are also observed in PO4ISR, where the average improvement (12.65\%) on ML-1M  is smaller than that (100.55\%) on Games. This demonstrates the advanced ability of LLMs to address the data sparsity issue. Lastly, our PO4ISR consistently achieves the best performance among all baselines, with an average improvement of 57.37\% and 61.03\% on HR and NDCG, respectively.   

\subsubsection{Ablation Study (RQ2)}
To verify the efficacy of different components, we compare PO4ISR with its four variants. In particular, `Initial' means we only use the initial prompt without optimization for each domain; `Top-1' means we merely adopt the Top-1 prompt within each domain; `EnSame' means we ensemble the ranking results of both Top-1 and -2 prompts within each domain; `EnCross' means we ensemble the ranking results of Top-1 prompts across all domains. The performance is shown in Table~\ref{tab:ablation}. 
Three observations are noted: (1) Initial performs worse than Top-1, which indicates the effectiveness of iterative prompt optimization; (2) both EnSame and EnCross underperform Top-1, implying that simply ensembling the top prompts either within the same domain or across different domains cannot efficiently improve the performance; and (3) PO4ISR with the Top-1 prompt in the games domain consistently achieves the best performance across all datasets, showcasing the efficacy of our cross-domain prompt selection strategy. This is further confirmed by Figure~\ref{fig:cross-domain}, presenting the performance of Top-1 prompt from each domain in the cross-domain scenario.   


\subsubsection{Parameter Analysis (RQ3)}
We further investigate the impact of important hyperparameters on PO4ISR. 
First, we examine the impact of different initial prompts. To this end, we substitute the initial task description (Prompt 1) with Prompt 9 incorporating two major changes: (1) we use `preferences' to replace `intentions', and the two terms have the same meanings in the context of ISR, and (2) we simplify the four subtasks into two subtasks.   
The results are presented in Table~\ref{tab:parameter-analysis} (rows 1-3 vs. rows 4-6), where we note that directly using Prompt 9 achieves better performance than using Prompt 1; meanwhile, the corresponding Top-1 prompt optimized based on Prompt 9 outperforms the Top-1 prompt optimized based on Prompt 1. This indicates that (1) simplified descriptions and subtasks division can improve the quality of the initial prompt, \textit{vice versa}; 
(2) the quality of the initial prompts positively affects the final performance; 
(3) regardless of the quality of initial prompts, they can be largely enhanced with iterative optimization; (4) the lower-quality initial prompt yields larger overall improvements;   
and (5) the performance of PO4ISR presented in Table~\ref{tab:comparison} is not the upper bound, and can be further improved with better initial prompts, showcasing its great potential. 
Besides, we study the impact of batch size $N_t$ on the final performance by varying its values in $\{16, 32\}$, and the results are presented in Table~\ref{tab:parameter-analysis} (row 2 vs. row 7). Accordingly, we find that $N_t=32$ is the optimal setting. 


\input{plot/prompt-initial-1}

\subsubsection{Visualization (RQ4)} To illustrate the results generated by PO4ISR, we randomly sample one test session from Bundle as shown in Figure~\ref{fig:case-study}. Given the historical session, PO4ISR first detects four combinations of items, including $[i_1, i_2, i_8], [i_3, i_4, i_6], [i_5, i_7], [i_9]$. The corresponding intents for each combination are (1) "this combination includes gummi bears, chamomile tea, and rosehip with hibiscus tea; the user might be interested in snacks and beverages for relaxation or enjoyment"; (2) "this combination includes organic infant formula, organic baby food, and organic baby food pouches; the user's intent seems to be focused on organic and healthy options for infants"; (3) "this combination includes Sriracha hot sauce and green hot sauce; the user's intent appears to be related to spicy condiments or sauces" and (4) "this combination includes green superfood capsules; the user's intent might be to explore or maintain a healthy lifestyle". Then it identifies and outputs the most important intent: 
"based on the given combinations, the intent related to organic and healthy options for infants (Combination 2) seems to be the most specific and focused". Finally, it furnishes a re-ranked recommendation list, positioning the ground truth item "Earth's Best Organic Baby Food, Spaghetti With Cheese" (highlighted in a red-dot circle) from its initial 11th rank within the candidate set to the topmost position. In summary, the case study validates that PO4ISR can help provide more comprehensible recommendations. 

\input{plot/parameter-analysis}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{image/case-study-1.png}
    \vspace{-0.1in}
    \caption{The case study on Bundle.}
    \label{fig:case-study}
    \vspace{-0.1in}
\end{figure}

\subsubsection{Discussion on Hallucination (RQ5)} 
%Despite the success of PO4ISR on the SR task, it showcases limitations due to the inherent issue of LLMs. One issue is the hallucination. Specifically, PO4ISR may generate some bad cases (e.g., the response does not contain the ranking list or the ground truth item is not included in the ranking list), although we add hard constraints in the prompt as "\textit{the order of all items in the candidate set must be provided, and the items for ranking must be within the candidate set}". Table~\ref{tab:bad-case} illustrates the ratio of bad cases on the test sets using the Top-1 prompt from each domain across the three datasets. Two major observations can be noted. 

Despite the success of PO4ISR on the SR task, it showcases limitations due to the inherent issue of LLMs. One issue is that PO4ISR may generate hallucination for some sessions (e.g., the response does not contain the ranking list or the ground truth item is not included in the ranking list), although we add hard constraints in the prompt such as "\textit{the order of all items in the candidate set must be provided, and the items for ranking must be within the candidate set}". Table~\ref{tab:bad-case} illustrates the ratio of sessions having hallucinations on the test sets using the Top-1 prompt from each domain across the three datasets. Two major observations can be noted. 
%
%
\textbf{(1)} The ratio is at its lowest on ML-1M but peaks on Bundle (emphasized in blue). This discrepancy likely stems from ML-1M having the highest average repeat frequency of items across sessions, whereas Bundle exhibits the lowest trend (see Table~\ref{tab:statistics}). The frequent appearance of items in various sessions may simplify the pattern recognition process, thus reducing task complexity to some extent. Additionally, Bundle's diverse range of electronics, clothing, and food products elevates the complexity of the SR task compared to the more focused ML-1M dataset. \textbf{(2)} The optimal prompts from different domains show comparable performance as highlighted in pink. On average, there are around 5.55\% sessions with hallucination, 
%(the baseline NIR has around 36\% of such sessions), 
implying that further performance enhancements can be obtained by addressing this issue and exhibiting the latent potential of LLMs for SR (note that the HR and NDCG values are set as 0 for sessions with hallucination).            
%

To this end, we involve JSON mode\footnote{\url{https://platform.openai.com/docs/guides/text-generation/json-mode}} in the response to better control the output by adding the constraint as \textit{Provide the ranking results for the candidate set using JSON format, following this format without deviation: [{"Item ID": "correspond item index", "Item Title": "correspond Item Title"}]}.
Table~\ref{tab:json} illustrates the performance contrast of PO4ISR on Bundle, with and without the JSON mode in the response. The results indicate that employing JSON mode marginally reduces bad cases, yet significantly compromises recommendation accuracy.
Contrarily, we find most such cases can be effectively resolved by using GPT-4 with improved accuracy. 
%Meanwhile, our utilization of GPT-4 on these cases demonstrates its ability to effectively resolve the majority of such instances with improved accuracy.
%
\input{plot/bad-cases}
\input{plot/json}






==> section/experiment.tex <==
\section{Experiments and Results}

\input{plot/data-statistic}

\input{plot/comparison}

\subsection{Experimental Setup}
\subsubsection{Datasets}
We adopt three real-world datasets from various domains. In particular, MovieLen-1M (ML-1M)\footnote{\url{https://grouplens.org/datasets/movielens/}} contains users' ratings of movies. Games is one subcategory from the Amazon dataset~\cite{ni2019justifying}, which contains users' ratings towards various games. Bundle~\cite{sun2022revisiting} is the human-labeled session data for three subcategories (Electronic, Clothing, and Food) of Amazon, where the item combination and the corresponding intents are annotated via crowdsourcing workers for each session. Table~\ref{tab:statistics} shows the statistics of the datasets.
For ML-1M and Games, we chronologically order the rated items into a sequence for each user and then divide it into sessions by day. For each dataset, we split the sessions into training, validation, and test sets with a ratio of 8:1:1, i.e., 80\% of the initial sessions are treated as training sets; the subsequent 10\% as the validation set; and the final 10\% as the test set.  


\subsubsection{Baselines} We compare our proposed paradigm with 10 baselines. They can be classified into three types. The first type is the conventional methods, including \textbf{Mostpop}: recommending the most popular items; \textbf{SKNN}~\cite{jannach2017recurrent}: recommending session-level similar items; and
\textbf{FPMC}~\cite{rendle2010factorizing}: the matrix factorization method with the first-order Markov chain.
%
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Mostpop}: recommending the most popular items;
%     \item \textbf{SKNN}~\cite{jannach2017recurrent}: recommending session-level similar items;
%     \item \textbf{FPMC}~\cite{rendle2010factorizing}: the matrix factorization method with the first-order Markov chain.
% \end{itemize}
%
The second type is the deep learning-based methods, which can be categorized into single intent based ones,
\textbf{NARM}~\cite{li2017neural}: an RNN-based model with the attention mechanism to capture the main purpose from the hidden states;
\textbf{STAMP}~\cite{liu2018stamp}: learning the general intention of users by emphasizing the effect of the last item in the context; and
\textbf{GCN-GNN}~\cite{wang2020global}: using both local and global graphs to learn item representation thus obtaining the main intent of the session;
%
% \begin{itemize}[leftmargin=*]
%     \item \textbf{NARM}~\cite{li2017neural}: an RNN-based model with the attention mechanism to capture the main purpose from the hidden states;
%     \item \textbf{STAMP}~\cite{liu2018stamp}: learning the general intention of users by emphasizing the effect of the last item in the context; 
%     \item \textbf{GCN-GNN}~\cite{wang2020global}: using both local and global graphs to learn item representation thus obtaining the main intent of the session;
% \end{itemize}
%
and multiple intent based models, 
\textbf{MCPRN}~\cite{wang2019modeling}: modeling users’ multiple purposes to get the final session representation; 
\textbf{HIDE}~\cite{li2022enhancing}: splitting the item embedding into multiple chunks, with each chunk representing a specific intention to learn diverse intentions within context;
and \textbf{Atten-Mixer}~\cite{zhang2023efficiently}: learning multi-granularity consecutive user intent units to generate more accurate session representations.
%
% \begin{itemize}[leftmargin=*]
%     \item \textbf{MCPRN}~\cite{wang2019modeling}: modeling users’ multiple purposes to get the final session representation; 
%     \item \textbf{HIDE}~\cite{li2022enhancing}: splitting the item embedding into multiple chunks, with each chunk representing a specific intention to learn diverse intentions within context;
%     \item \textbf{Atten-Mixer}~\cite{zhang2023efficiently}: learning multi-granularity consecutive user intent units to generate more accurate session representations.
% \end{itemize}
%
The last type is the LLM-based method
\textbf{NIR}~\cite{wang2023zero}: adopting zero-shot prompting for the next item recommendation.
%
% \begin{itemize}[leftmargin=*]
%     \item \textbf{NIR}~\cite{wang2023zero}: adopting zero-shot prompting for the next item recommendation.
% \end{itemize}
%

% \subsubsection{Evaluation Metrics}
% Following state-of-the-arts~\cite{yin2023understanding,wang2019modeling,wang2023zero}, we adopt HR@K and NDCG@K as the evaluation metrics with K=1/5/10. Generally, higher metric values indicate better ranking results. 
% For a more robust performance, we test each method five times and report the average results. 
 
%\input{plot/parameter}

\subsubsection{Parameter Settings}
We use %the open-source hyperparameter optimization framework 
Optuna (\url{optuna.org}) %\footnote{\url{https://optuna.org/}} 
to automatically find out the optimal hyperparameters of all methods with 30 trails.
In particular, the maximum training epoch is set as 100 with the early stop mechanism. 
The search space for item embedding size, learning rate, and batch size are 
$\{32,64,128\}$, $\{10^{-4},10^{-3},10^{-2}\}$ and $\{64,128,256\}$, respectively.    
For SKNN, $K$ is searched from $\{50,100,150\}$. 
For NARM, the hidden size and layers are searched in $[50, 200]$ stepped by 50 and in $\{1,2,3\}$, respectively.
For GCE-GNN, the number of hops, and the dropout rate for global and local aggregators are respectively searched in $\{1,2\}, [0, 0.8]$ stepped by 0.2, and $\{0, 0.5\}$.  
For MCPRN, $\tau$ and the number of purpose channels are separately searched in $\{0.01, 0.1, 1, 10\}$ and $\{1,2,3,4\}$.
For HIDE, the number of factors is searched in $\{1,3,5,7,9\}$; the regularization and balance weights are searched in $\{10^{-5},10^{-4},10^{-3},10^{-2}\}$; the window size is searched in $[1,10]$ stepped by 1; and the sparsity coefficient is set as 0.4.
For Atten-Mixer, the intent level $L$ and the number of attention heads are respectively searched in $[1,10]$ stepped by 1 and in $\{1,2,4,8\}$.
%
For PO4ISR, $N=50, N_t=N_v=32, N_r=2, N_o=4, E_1=16, E_2=2$; and
we randomly select 8 prompts as the input of the UCB Bandits in each iteration. 

Following state-of-the-arts~\cite{yin2023understanding,wang2019modeling,wang2023zero}, we adopt HR@K and NDCG@K as the evaluation metrics with K=1/5. Generally, higher metric values indicate better ranking results. Note that the candidate size of all methods is set as 20.
For a fair comparison, all baselines are trained with 150 randomly sampled sessions from the training set; to manage the API call cost, for ML-1M and Games, we randomly sample 1000 sessions from the validation set and test set, respectively. For robust performance, we repeat the test procedure five times and report the average results\footnote{Our code and data are available at \url{https://www.xxxxx.xxxx}}.

\input{plot/ablation}
\input{plot/cross-domain-test}


\subsection{Results and Analysis}

\subsubsection{Overall Comparison}

Table~\ref{tab:comparison} presents the performance of all methods on the three datasets. Several major findings are noted. 

\textbf{(1)} Regarding conventional methods (CMs), the model-based FPMC performs the best on sparser datasets Games and Bundles, while is slightly defeated by SKNN on the denser dataset ML-1M (see `Avg. Item Repeat Frequency' in Table~\ref{tab:statistics} where higher average repeat frequency of items across sessions indicates larger density, \textit{vice versa}). This exhibits the strong capability of the model-based method in learning the sequential patterns under the data sparsity scenario. \textbf{(2)} For single-intent methods (SIMs), each gains its best performance on different datasets, e.g., NARM excels on ML-1M, whereas GCE-GNN wins on Games. Generally, GCE-GNN showcases advantages on shorter sessions with sparser datasets (e.g., Games). This is because such sessions do not contain sufficient local information, thus requiring global information (graph) to compensate. Conversely, NARM performs well on longer sessions with denser datasets (e.g., ML-1M). These longer sessions possess substantial information and frequent patterns, making the fusion of global information potentially noisy. \textbf{(3)} With regard to multi-intent methods (MIMs), MCPRN displays the poorest performance across all datasets, as limited training data hinders the learning of appropriate parameters for multiple RNN channels. Besides, HIDE exceeds Atten-Mixer on relatively denser datasets (ML-1M and Games) but lags behind Atten-Mixer on the sparsest dataset Bundle.
\textbf{(4)} Among LLM-based methods (LLMMs), PO4ISR outperforms NIR, corroborating our prior assertion that basic in-context learning fails to fully exploit LLMs, thereby emphasizing the superiority of our prompt optimization paradigm.  

Overall, CMs underperform SIMs or MIMs, underscoring the importance of capturing user intents for improved SR. The victory of MIMs over SIMs on Bundle validates the effectiveness of multi-intent learning. However, some of the SIMs (e.g., NARM) surpass MIMs (e.g., MCPRN) on ML-1M and Games, suggesting that fixed numbers of intents might constrain the capability of MIMs. LLMMs exhibit strength on sparser datasets compared to denser ones (e.g., NIR on Games vs. ML-1M), and shorter sessions compared to longer ones (e.g., NIR on Games vs. Bundles). Similar trends are also observed in PO4ISR, where the average improvement (12.65\%) on ML-1M  is smaller than that (100.55\%) on Games. This demonstrates the advanced ability of LLMs to address the data sparsity issue. Lastly, our PO4ISR consistently achieves the best performance among all baselines, with an average improvement of 57.37\% and 61.03\% on HR and NDCG, respectively.   

%\begin{itemize}
%\item The same training samples with the proposed method (150) are shown in Table~\ref{tab:comparison} (\ding{52})
%\item The number of samples to reach the same results as the proposed method shown in Table~\ref{tab:sample-number} (\textcolor{red}{change as figures with three points 50, 150, and 10000})
%\end{itemize}

%\noindent The proposed method
% \begin{itemize}
%     %\item Cross-domain test shown in Table~\ref{tab:comparison} (\ding{52})
%     \item Cross-domain to verify the generalization of the proposed method (shown in Figure~\ref{fig:cross-domain}) (\ding{52})
% \end{itemize}

%Dense data -> perform worse;
%Sparse data -> perform better; 


\subsubsection{Ablation Study}
To verify the efficacy of different components, we compare PO4ISR with its four variants. In particular, `Initial' means we only use the initial prompt without optimization for each domain; `Top-1' means we merely adopt the Top-1 prompt for each domain; `EnSame' means we ensemble the ranking results of both Top-1 and -2 prompts within each domain; `EnCross' means we ensemble the ranking results of Top-1 prompts across all domains. The performance is shown in Table~\ref{tab:ablation}. 
Three observations are noted: (1) Initial performs worse than Top-1, which indicates the effectiveness of iterative prompt optimization; (2) both EnSame and EnCross underperform Top-1, implying that simply ensembling the top prompts either within the same domain or across different domains cannot efficiently improve the performance; and (3) PO4ISR with the Top-1 prompt in the games domain consistently achieves the best performance across all datasets, showcasing the efficacy of our prompt curation strategy. This can be further confirmed by Figure~\ref{fig:cross-domain}, which presents the performance of Top-1 prompt from each domain in the cross-domain scenario.   


%Cross-domain to verify the generalization of the proposed method (shown in Figure~\ref{fig:cross-domain}) (\ding{52})

% \begin{itemize}
%     \item only with initial prompts  (initial)
%     \item only with the top-1 prompt (top-1)
%     \item simply ensemble top-1 and -2 prompts within the same domain (EnSame)
%     \item simply ensemble the top-1 prompts across different domains (EnCross)
% \end{itemize}


\subsubsection{Parameter Analysis}
We further investigate the impact of important hyperparameters.
First, we examine the impact of different initial prompts. To this end, we replace the initial task description prompt (Prompt 1) with Prompt 9. The results are presented in Table~\ref{tab:parameter-analysis} (rows 1-3 vs. rows 4-6), where we note that directly using Prompt 9 achieves better performance than using Prompt 1; meanwhile, the corresponding Top-1 prompt optimized based on Prompt 9 outperforms the Top-1 prompt optimized based on Prompt 1. This indicates that (1) the quality of the initial prompts positively affect the final performance; (2) regardless of the quality of initial prompts, they can be largely enhanced with the iterative optimization; (3) the lower-quality initial prompt yields   larger overall improvements; and (4) the performance of PO4ISR presented in Table~\ref{tab:comparison} are not the upper bound, and can be further improve with better inital prompts, showcasing its great potential. 
Besides, we study the impact of batch size $N_t$ on the final performance by varying its values in $\{16, 32\}$, and the results are presented in Table~\ref{tab:parameter-analysis} (row 2 vs. row 7). Accordingly, we find that $N_t=32$ is the optimal setting. 


\input{plot/prompt-initial-1}

\input{plot/parameter-analysis}



%\noindent Parameter Analysis on Bundle (\ding{52})
% \begin{itemize}
%     \item different initial prompts
%     \item batch\_size [16, 32]
% \end{itemize}


% \begin{itemize}
%     \item Conduct a case study to visualize the generated intents and recommendations; %and compare the number of generated intents of different methods
% \end{itemize}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{image/case-study.png}
    \vspace{-0.1in}
    \caption{The case study on Bundle.}
    \label{fig:case-study}
    \vspace{-0.1in}
\end{figure}


\subsubsection{Visualization} To further illustrate the results generated by PO4ISR, we randomly sample one test session from Bundle as shown in Figure~\ref{fig:case-study}. Given the historical session, PO4ISR first detects four combinations of items, including $[i_1, i_2, i_8], [i_3, i_4, i_6], [i_5, i_7], [i_9]$. The corresponding intents for each combination are (1) "this combination includes gummi bears, chamomile tea, and rosehip with hibiscus tea; the user might be interested in snacks and beverages for relaxation or enjoyment"; (2) "this combination includes organic infant formula, organic baby food, and organic baby food pouches; the user's intent seems to be focused on organic and healthy options for infants"; (3) "this combination includes Sriracha hot sauce and green hot sauce; the user's intent appears to be related to spicy condiments or sauces" and (4) "this combination includes green superfood capsules; the user's intent might be to explore or maintain a healthy lifestyle". Then it identifies and outputs the most important intent: 
"based on the given combinations, the intent related to organic and healthy options for infants (Combination 2) seems to be the most specific and focused". %"Considering the user's personalized information, it is important to prioritize the intent that aligns with their individual tastes, dietary restrictions, and other relevant factors. Without specific information about the user's preferences, it is difficult to determine the most representative intent. However, based on the given combinations, the intent related to organic and healthy options for infants (Combination 2) seems to be the most specific and focused". 
Finally, it furnishes a reranked recommendation list, positioning the ground truth item "Earth's Best Organic Baby Food, Spaghetti With Cheese" from its initial 11th rank within the candidate set to the topmost position.



\subsubsection{Discussion on Hallucination} 
Despite the success of PO4ISR on the SR task, it showcases limitations due to the inherent issue of LLMs. One issue is the hallucination. Specifically, PO4ISR may generate some bad cases (e.g., the response does not contain the ranking list or the ground truth item is not included in the ranking list), although we add hard constraints in the prompt as "\textit{the order of all items in the candidate set must be provided, and the items for ranking must be within the candidate set}". Table~\ref{tab:bad-case} illustrates the ratio of bad cases on the test sets using the Top-1 prompt from each domain across the three datasets. Two major observations can be noted. 
%
\textbf{(1)} The ratio is at its lowest on ML-1M but peaks on Bundle (emphasized in blue). This discrepancy likely stems from ML-1M having the highest average repeat frequency of items across sessions, whereas Bundle exhibits the lowest trend (see Table~\ref{tab:statistics}). The frequent appearance of items in various sessions simplifies pattern recognition, somewhat reducing task complexity. Additionally, Bundle's diverse range of electronics, clothing, and food products elevates the complexity of the SR task compared to the more focused ML-1M dataset. \textbf{(2)} The optimal prompts from different domains show comparable performance as highlighted in pink. On average, there are around 5.55\% bad cases, implying that further performance enhancements can be obtained by addressing these cases, and exhibiting the latent potential of LLMs for SR.            
%
%\input{plot/bad-case}
%
%\begin{itemize}
    % \item Discuss the bad cases as shown in Table~\ref{tab:bad-case} (\ding{52})
    % \item Impact of JSON format and its reasons in Table~\ref{tab:json} (\ding{52})
%\end{itemize}

To ease this issue, we try to involve the JSON mode\footnote{\url{https://platform.openai.com/docs/guides/text-generation/json-mode}} in the response to better control the output. 
Table~\ref{tab:json} illustrates the performance contrast of PO4ISR on Bundle, with and without the JSON mode in the response. The results indicate that employing JSON mode marginally reduces bad cases, yet significantly compromises recommendation accuracy. Meanwhile, our utilization of GPT-4 on these cases demonstrates its ability to effectively resolve the majority of such instances with improved accuracy.
x
\input{plot/bad-cases}
\input{plot/json}






==> section/intro-v2.tex <==
\section{Introduction}
Session-based recommendation (SR)~\cite{lai2022attribute,chen2022autogsr,han2022multi,hou2022core,yang2023loam} aims to predict the next interacted item based on short anonymous behavior sessions. 
%
Typically, different sessions may unveil diverse user intents~\cite{wang2019modeling}. Figure~\ref{fig:intent-example} illustrates two real sessions in Amazon Electronic dataset~\cite{ni2019justifying}, where the first session %shown
in (a) reflects one main purpose, i.e., shopping for laptop and accessories, whereas the second one %depicted
in (b) is associated with two major intents, i.e., shopping for laptop protectors and camera accessories, respectively. 
However, most public datasets do not include explicit intents of a session as it may be intrusive and disruptive to ask users about their current session purposes directly~\cite{oh2022implicit}.
Hence, intent-aware session recommendation (ISR) has emerged to capture the latent user intents within a session, thus enhancing the accuracy of SR.

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{image/Intent-Example.pdf}
    \vspace{-0.1in}
    \caption{Examples of user sessions with various intents.}
    \label{fig:intent-example}
    \vspace{-0.15in}
\end{figure}

Specifically, early studies in ISR~\cite{li2017neural,liu2018stamp,wang2020global} primarily
%generate recommendations by constraining 
constrain sessions to a single purpose or goal, such as shopping for a laptop and accessories in Figure~\ref{fig:intent-example}(a). However, this simplistic assumption doesn't always hold in real-world scenarios, where a session may involve diverse items
for various purposes, as illustrated in Figure~\ref{fig:intent-example}(b). It thus poses barriers for such methods seeking further performance improvements. Consequently, various approaches have been developed to model multiple intentions within a session, e.g., IDSR~\cite{chen2020improving}, MCPRN~\cite{wang2019modeling}, and NirGNN~\cite{jin2023dual}. Despite the success, they suffer from two major limitations. First, they rely on an unrealistic assumption that all sessions possess a consistent and fixed number of intentions, treating this as a hyper-parameter. Second, they are limited to learning latent intentions solely within the embedding space, greatly impeding the transparency of ISR. Such limitations thus further hinder these approaches from delivering more accurate and comprehensible recommendations.

Fortunately, the rise of large language models (LLMs) has opened up unprecedented opportunities in the field of ISR. LLMs, armed with advanced reasoning capabilities, have found widespread application in general recommendation scenario~\cite{dai2023uncovering,he2023large,sanner2023large,bao2023tallrec}, but have been relatively underexplored in the context of SR. In the limited body of research on SR, LLMs are generally employed in two distinct ways, namely in-context learning (ICL)~\cite{wang2023zero,hou2023large} and parameter-efficient fine-tuning~\cite{bao2023bi,yue2023llamaRec}. 
However, LLMs cannot fully realize their potential through simple ICL (e.g., zero-shot prompting~\cite{wang2023zero}). While fine-tuning LLMs holds promise, it grapples with challenges stemming from computational demands and the availability of open-source LLMs. %Furthermore, these methods often fall short in exploiting the capabilities of LLMs to comprehend user intents at the semantic level, a vital aspect for enhancing the efficacy of SR. 

Therefore, we propose a simple yet effective paradigm to exploit the power of LLMs for more effective ISR from the perspective of prompt optimization (abbreviated as PO4ISR). 
It is equipped with Prompt Initialization (\textit{PromptInit}), Prompt Optimization (\textit{PromptOpt}), and Prompt Selection (\textit{PromptSel}). In particular, PromptInit aims to create an initial prompt that guides LLMs to dynamically understand session-level user intents, and predict the next item accordingly. 
Inspired by the study on automatic prompt optimization~\cite{pryzant2023automatic} in natural language processing (NLP), PromptOpt
seeks to automatically optimize the initial prompt with self-reflection. To be specific, the LLM is required to offer reasoning rooted in the identified errors to improve (refine and augment) the initial prompt. The performance of improved prompts is then assessed with UCB bandits~\cite{audibert2010best}, thereby helping shortlist promising prompt candidates for an iterative optimization. 
Lastly, PromptSel prioritizes the selection of optimized prompts by harnessing the robust generalizability of LLMs across diverse domains, aiming to maximize accuracy improvements.
As such, PO4ISR can efficiently direct LLMs to infer and comprehend dynamic user intents at a semantic level, resulting in more accurate and understandable SR. 

\medskip\noindent\textbf{Contributions}. Our main contributions lie three-fold. \textbf{(1)} We introduce a simple yet powerful paradigm -- PO4ISR-- to harness the capabilities of LLMs for enhanced ISR through prompt optimization. \textbf{(2)} The PO4ISR paradigm, composed of prompt initialization, optimization, and selection modules, empowers LLMs to semantically comprehend varying user intents in a session, resulting in more accurate and comprehensible SR. \textbf{(3)} Experiments on real-world datasets demonstrate that PO4ISR significantly outperforms baselines with an average improvement of 57.37\% and 61.03\% on HR and NDCG, respectively.   
Meanwhile, several insightful observations are gained, for example, 
(a) PO4ISR yields promising accuracy with only a small number of training samples; 
(b) PO4ISR exhibits advanced generalizability and excels in cross-domain scenarios;  
(c) PO4ISR showcases superior strength on sparser datasets with shorter sessions compared; however, it might exhibit increased hallucination tendencies with sparser datasets; (d) the performance of PO4ISR shows a positive correlation with the quality of the initial prompt, and lower-quality initial prompts tend to yield more significant improvements; and (f) a streamlined description and subtask division can enhance the quality of initial prompts.

==> section/intro.tex <==
\section{Introduction}
Session-based recommendation (SR)~\cite{lai2022attribute,chen2022autogsr,han2022multi,hou2022core,yang2023loam} aims to predict the next interacted item based on short anonymous behavior sessions. 
%
Typically, different sessions may unveil diverse user intents~\cite{wang2019modeling}. Figure~\ref{fig:intent-example} illustrates two real sessions in Amazon Electronic dataset~\cite{ni2019justifying}, where the first session %shown
in (a) reflects one main purpose, i.e., shopping for laptop and accessories, whereas the second one %depicted
in (b) is associated with two major intents, i.e., shopping for laptop protectors and camera accessories, respectively. 
However, most public datasets do not include explicit intents of a session as it may be intrusive and disruptive to ask users about their current session purposes directly~\cite{oh2022implicit}.
Hence, intent-aware session recommendation (ISR) has emerged to capture the latent user intents within a session, thus enhancing the accuracy of SR.

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{image/Intent-Example.pdf}
    \vspace{-0.1in}
    \caption{Examples of user sessions with various intents.}
    \label{fig:intent-example}
    \vspace{-0.15in}
\end{figure}

Early studies in ISR~\cite{li2017neural,liu2018stamp,wang2020global} %primarily
generate recommendations by constraining sessions to a single purpose or goal, such as shopping for a laptop and accessories in Figure~\ref{fig:intent-example}(a). However, this simplistic assumption doesn't always hold in real-world scenarios, where a session can involve 
%a diverse array of items 
diverse items
for various purposes, as illustrated in Figure~\ref{fig:intent-example}(b). It thus poses barriers for single-intent based methods seeking to attain further performance improvements. Consequently, various approaches have been developed to model multiple intentions within a session, e.g., NirGNN~\cite{jin2023dual}, IDSR~\cite{chen2020improving}, MCPRN~\cite{wang2019modeling}, and HIDE~\cite{li2022enhancing}. Despite their successes, these methods suffer from two significant limitations. Firstly, they rely on an unrealistic assumption that all sessions possess a consistent and fixed number of intentions, treating this as a hyper-parameter. Secondly, they are limited to learning latent intentions solely within the embedding space, greatly impeding the transparency of the ISR. These issues further hinder current multi-intent approaches from delivering more accurate and interpretable recommendations.

Fortunately, the rise of large language models (LLMs) has opened up unprecedented opportunities %in the field of ISR.
for ISR.
Equipped with extensive knowledge and advanced logical reasoning capabilities, LLMs have found extensive use in general recommendation~\cite{dai2023uncovering,he2023large,sanner2023large,bao2023tallrec} but have been relatively underexplored in the context of SR.
In the limited body of research on SR, LLMs are generally employed in two distinct ways, namely in-context learning (ICL)~\cite{wang2023zero,hou2023large}, and fine-tuning~\cite{bao2023bi,yue2023llamaRec}. 
%
%Among the few studies on SR, LLMs are basically utilized in three manners, including zero-shot learning~\cite{wang2023zero}, in-context learning~\cite{hou2023large}, and fine-tuning~\cite{bao2023bi,yue2023llamaRec}. 
%
However, LLMs cannot fully realize their potential through simple ICL (e.g., zero-shot prompting~\cite{wang2023zero}). While fine-tuning LLMs holds promise, it grapples with challenges stemming from computational demands and the availability of open-source LLMs. Furthermore, these methods often fall short in exploiting the capabilities of LLMs to comprehend user intents at the semantic level, a vital aspect for enhancing the efficacy of SR. 

Therefore, we propose a simple yet effective paradigm to exploit the power of LLMs for more effective ISR from the perspective of prompt optimization (abbreviated as PO4ISR). 
It is equipped with Prompt Initialization (\textit{PromptInit}), Prompt Optimization (\textit{PromptOpt}), and Prompt Curation (\textit{PromptCura}). In particular, PromptInit aims to create an initial prompt that guides LLMs to dynamically understand session-level user intents, and predict the next item accordingly. 
Inspired by the study on automatic prompt optimization~\cite{pryzant2023automatic} in natural language processing (NLP), PromptOpt
seeks to automatically optimize the initial prompt with self-reflection. To be specific, the LLM is required to reconsider and offer justifications rooted in the identified errors to refine and augment the initial prompt. The performance of refined prompts is subsequently evaluated with UCB bandits~\cite{audibert2010best}. Afterwards, the beam search is employed to cherry-pick promising prompt candidates for iterative optimization.   
%
Lastly, PromptCura prioritizes the selection of optimized prompts for various sessions based on cross-domain performance to maximize the accuracy enhancements of SR.
In doing this, PO4ISR is capable of efficiently guiding LLMs to infer and understand dynamic user intents at the semantic level, thus delivering more accurate and transparent SR. 

\medskip\noindent\textbf{Contributions}. Our main contributions lie three-fold. \textbf{(1)} We introduce a simple yet powerful paradigm -- PO4ISR-- to harness the capabilities of LLMs for enhanced ISR, focusing on the optimization of prompts. \textbf{(2)}. The PO4ISR paradigm, composed of Prompt Initialization, Optimization, and Curation modules, empowers LLMs to semantically comprehend dynamic user intents in a session, resulting in more precise and interpretable outcomes. \textbf{(3)} Extensive experiments on three real-world datasets demonstrate that PO4ISR significantly outperforms baselines with an average improvement of 57.37\% and 61.03\% on HR and NDCG, respectively.   
Meanwhile, a number of insightful findings are gained, for example, 
(a) PO4ISR can yield optimal prompts and promising accuracy with only a small number of training samples; 
(b) PO4ISR exhibits advanced generalizability and excels in cross-domain scenarios;  
(c) PO4ISR showcases strength on sparser datasets with shorter sessions compared to denser datasets with longer sessions; however, it might exhibit increased hallucination tendencies with sparser datasets;
and (d) the performance of PO4ISR shows a positive correlation with the quality of the initial prompt; moreover, lower-quality initial prompts tend to yield more significant improvements.
%(4) PO4ISR aids in identifying a variable number of semantic intents within each session, enhancing the interpretability of recommendations;
%and
%(5) the JSON format data does not always improve the quality of the response of LLMs.




%\begin{itemize}
    %\item Definition of session-aware recommendation, and demonstrate different sessions may unveil different user intents
    %\item Existing intent-aware session recommendation approaches and their limitations, e.g., latent intents as hyper-parameters, thus less transparency;
    %\item Introducing large language models and their advantages for explainable session-aware recommendation
    %\item the challenges/issues faced, e.g., fine-tuning with high-cost
    %\item Present the overall framework and highlight important findings
    %\item Summarize the contribution
%\end{itemize}

%APO~\cite{pryzant2023automatic} 


==> section/method-v2.tex <==
\section{The Proposed Method}
This section introduces the PO4ISR paradigm, a simple yet powerful framework inspired by the work~\cite{pryzant2023automatic} in the area of NLP. It is specifically designed to efficiently guide LLMs in comprehending varying user intents at a semantic level, with the goal of enhancing the accuracy and transparency of SR.


\medskip\noindent\textbf{Framework Overview}.
Figure~\ref{fig:framework} illustrates the overall framework, mainly composed of three key components. Specifically, Prompt Initialization (\textit{PromptInit}) is tasked with generating an initial prompt that directs LLMs in dynamically comprehending semantic user intents at the session level within a session. Subsequently, Prompt Optimization (\textit{PromptOpt}) aims to evaluate, refine, augment, and optimize the initial prompt through self-reflection (i.e., inferring reasons from the collected error cases). Lastly, Prompt Selection (\textit{PromptSel}) is designed to properly select optimized prompts by exploiting the robust generalizability of LLMs across diverse domains, thus maximizing the accuracy enhancements of SR.

\subsection{Prompt Initialization (PromptInit)}\label{sec:prompt-initialization}
Given a session, we first create an initial prompt for the task description. It seeks to guide LLMs in understanding the varying user intents at the semantic level, which thus empowers LLMs to make more accurate and comprehensible recommendations. The task description is demonstrated in Prompt 1 which divides the SR task into four subtasks by using the planning strategy~\cite{zhou2023least}.
%
Then, Prompt 1 is used to guide ChatGPT\footnote{Without a further statement, it is based on GPT-3.5-turbo.} to predict the next item based on the historical (training) user sessions fed by Prompt 2. 
%
For ease of understanding, we take one training session as an example, that is, the current session interactions: [1."Zenana Women's Cami Sets", 2."Monster Tattoos", 3."I Love You This Much Funny T-rex Adult T-shirt", 4."Breaking Bad Men's Logo T-Shirt", 5."Sofia the First Sofia's Transforming Dress", 6."Lewis N. Clark 2-Pack Neon Leather Luggage Tag", 7."Russell Athletic Women's Stretch Capri", 8."US Traveler New Yorker 4 Piece Luggage Set Expandable", 9."Soffe Juniors Football Capri"]. The target (ground truth) item "It's You Babe Mini Cradle, Medium" is ranked at position 19 out of 20 items in the candidate set. After using the initial prompt, the target item holds the 16th position in the re-ranked candidate set. 

\subsection{Prompt Optimization (PromptOpt)}

PromptOpt strives to evaluate, refine, augment, and optimize the initial task description prompt with an iterative self-reflection. The detailed process is elaborated in what follows.

\medskip\noindent\textbf{Collecting Error Cases}. 
We randomly sample a batch ($N_t$) of sessions from training sessions ($N$) and guide ChatGPT to predict the next items with the initial prompts.
Afterwards, we evaluate the recommendation outcomes, considering sessions where the target item ranks in the bottom half of the re-ranked candidate set as error cases. Following this rule,  the example session mentioned in Section~\ref{sec:prompt-initialization} is an error case, since the ranking position of the target item by using the initial prompt is 16 out of 20 candidates. 
These error cases, indicating that the corresponding prompts do not effectively guide LLMs in performing the SR task, will be utilized to further refine the prompts. We use $N_e$ ($0\leq N_e \leq N_t$) to denote the total number of such error cases for each batch. 

\medskip\noindent\textbf{Inferring Reasons}. Understanding the reasons behind these collected error cases would greatly aid in refining the prompts, consequently enhancing recommendation performance. Thus, we leverage the self-reflection ability of ChatGPT, that is, asking ChatGPT to reconsider and offer justifications rooted in the identified errors. Inspired by~\cite{pryzant2023automatic}, we adopt Prompt 3 to generate $N_r$ reasons for each of the $N_e$ error cases, where the `\textit{error\_case}' includes the user session and candidate item set. 
%
Below demonstrates the generated reasons for one error case. 
%
\begin{itemize}[leftmargin=*]
\item \textit{One reason why the prompt could have gotten these examples wrong is that it assumes that the user's interactive intent can be accurately inferred based solely on the items within each combination. However, the prompt does not provide any information about the user's preferences, tastes, or previous interactions. Without this context, it is difficult to accurately infer the user's intent from the items alone.}
\item \textit{Another reason is that the prompt does not specify how the combinations of items within the session should be discovered. It assumes that the combinations are already known and provided as input. However, in real-world scenarios, discovering meaningful combinations of items from a user's session interactions can be a complex task. The prompt does not provide any guidance on how to perform this discovery process, which can lead to incorrect results. }   
\end{itemize}

\medskip\noindent\textbf{Refining Prompts}. With the inferred $N_r$ reasons for each error case, we now ask ChatGPT to refine the current prompt accordingly using Prompt 4. One example of the refined prompt is illustrated as Prompt 5. 
By comparing the initial task description (Prompt 1) and the refined Prompt 5, we can easily note that the initial prompt is improved by considering two aspects: (1) user preference and taste and (2) the definition of item combinations. These two aspects are exactly consistent with the inferred reasons by ChatGPT. 

\medskip\noindent\textbf{Augmenting Prompts}. With the refined prompts, we further ask ChatGPT to augment prompts (Prompt 7 is an example of augmentation) with the same semantic meanings using Prompt 6. Accordingly, for the $N_e$ error cases, we finally obtain $2N_e$ improved prompts through refinement and augmentation. These prompts will be further utilized for an iterative optimization based on their recommendation performance, as introduced in what follows. 

\medskip\noindent\textbf{Evaluating Prompts}.
From the pool of $2N_e$ prompts, identifying the most efficient ones with the best recommendation accuracy is crucial. One greedy way is to evaluate their performance with all historical user sessions. However, this may be quite computationally expensive. To improve the efficiency, we employ the upper confidence bound (UCB) Bandits~\cite{pryzant2023automatic} to efficiently estimate the performance. In particular, it iteratively samples one prompt based on its estimated performance and then evaluates the prompt on a random batch of training sessions ($N_t$), and finally updates its performance based on the observed performance. The process is depicted by Algorithm~\ref{alg:ucb}, where the reward is calculated by the NDCG measuring the ranking position of the target item; and $\gamma$ is the exploration parameter. With UCB Bandits, we can quickly obtain the estimated performance of the $2N_e$ prompts.

% 
\input{plot/prompt-task}
\input{plot/prompts-input}
\input{plot/prompt-reason}
\input{plot/prompt-refine}
%


\medskip\noindent\textbf{Iterative Optimization}. 
Based on UCB Bandits, we then iteratively optimize the prompts~\cite{pryzant2023automatic}. According to the estimated performance $R$, we select the Top-$N_o$ prompts and carry these promising prompts forward to the subsequent iteration. Specifically, we first use the Top-$N_o$ prompts to replace the prompts in the previous iteration, and then conduct the series of tasks, i.e., collecting error cases, inferring reasons, refining, augmenting, and evaluating prompts, as described in Algorithm~\ref{alg:beam-search}. 
This iterative loop fosters incremental enhancements and exploration among various promising prompt candidates.  
%
Prompt 8 is an example of an optimized prompt with the best-estimated performance in the final iteration. After applying it on the example session mentioned in Section~\ref{sec:prompt-initialization}, the target item has been re-ranked to the 11th position, advancing eight positions from its previous placement in the candidate set.   

%
\input{plot/out-improve}
\input{plot/prompt-augment}
\input{plot/out-augment}
\input{plot/out-optimal}

\input{plot/ucb}

\input{plot/beam-search}


\subsection{Prompt Selection (PromptSel)}
At the end of the iterative optimization, we have the Top-$N_o$ prompts. Accordingly, one straightforward way is to choose the Top-1 prompt as the final selection due to its superior overall performance. However, we notice that although a majority of sessions achieve their peak accuracy with the Top-1 prompt, a subset of them displays the best performance with other Top prompts. This can be verified by Figure~\ref{fig:same-domain-prompt}, which shows the performance gap between the Top-1 and Top-2 prompts on the validation sessions across three real-world datasets in the domains of movie, games, and e-commerce (with bundled products)\footnote{The details of the datasets utilized in our study are introduced in Section 4.1.1.}. 
From the results, it's evident that there are data points positioned where the gap is less than zero, signifying that the Top-2 prompt surpasses the Top-1 prompt in some cases. 
%
Thus, one can come up with potential solutions: (1) ensemble all top prompts to get the compensation results; and (2) train a classifier to select the best top prompt for each session. 
Nevertheless, we empirically discovered that (1) fails to yield promising results because the enhancements in the subset do not offset the declines in the majority; while (2) heavily relies on the accuracy of the classifier, thus bringing in extra uncertainty to the final performance. 

\input{plot/same-domain-validation}
\input{plot/cross-domain-validation}

Fortunately, the robust generalizability of LLMs inspires us to explore the cross-domain performance of these optimized prompts. Specifically, Figure~\ref{fig:cross-domain-validation} depicts the performance of the Top-1 prompts from the three domains across the three datasets, for instance, `Opt-Games' (in purple) refers to the Top-1 prompt in the games domain. From the figure, we can easily notice that Opt-Games consistently performs the best not only in its games domain but also in the other two domains. One possible explanation could be attributed to the Games dataset having the shortest average session length (refer to the `Avg. Session Length' in Table~\ref{tab:statistics}) alongside a moderate level of sparsity (see `Density Indicator' in Table~\ref{tab:statistics}). These factors collectively alleviate the challenge of identifying the optimal prompt to capture crucial and unique information, thereby enhancing the overall performance of SR.
Accordingly, we select the Opt-Games as the final prompt for all domains, the efficacy of which is verified in Section 4.2.  





==> section/method.tex <==
\section{The Proposed Method}
This section introduces the PO4ISR paradigm, a simple yet powerful framework inspired by the work~\cite{pryzant2023automatic} in the area of NLP. It is specifically designed to efficiently guide LLMs in comprehending dynamic user intents at a semantic level, with the goal of enhancing the precision and transparency of SR.


\medskip\noindent\textbf{Framework Overview}.
Figure~\ref{fig:framework} illustrates the overall framework, mainly composed of three key components. Specifically, the Prompt Initialization (\textit{PromptInit}) module is tasked with generating an initial prompt aimed at guiding LLMs in dynamically comprehending semantic user intents at the session level. Subsequently, the Prompt Optimization (\textit{PromptOpt}) module focuses on augmenting, refining, and optimizing the initial prompt through self-reflection. Lastly, the Prompt Curation (\textit{PromptCura}) module is dedicated to selecting and assigning appropriate optimized prompts for various sessions using the Gaussian Navia Bayes classifier, thus maximizing the performance enhancements of SR.

\subsection{Prompt Initialization (PromptInit)}\label{sec:prompt-initialization}
Given a session, we first create an initial prompt for the task description. It seeks to guide LLMs in understanding the dynamic user intents at the semantic level, which thus empowers LLMs to make more accurate and transparent recommendations. The task description is demonstrated in Prompt 1 which divides the SR task into four subtasks by using the planning strategy~\cite{zhou2023least}.
%
The task description prompt is then used to guide ChatGPT\footnote{Without a further statement, it is based on GPT-3.5-turbo.} with the role of `system'. Meanwhile, we create another prompt (see Prompt 2) to input the user session and item candidates into the ChatGPT designated under the 'user' role.

With these initial prompts, we can instruct ChatGPT to generate next item recommendations based on the
historical (training) user sessions. For ease of understanding, we take one training session as an example, that is, Current session interactions: [1."Zenana Women's Cami Sets", 2."Monster Tattoos", 3."I Love You This Much Funny T-rex Adult T-shirt", 4."Breaking Bad Men's Logo T-Shirt", 5."Sofia the First Sofia's Transforming Dress", 6."Lewis N. Clark 2-Pack Neon Leather Luggage Tag", 7."Russell Athletic Women's Stretch Capri", 8."US Traveler New Yorker 4 Piece Luggage Set Expandable", 9."Soffe Juniors Football Capri"]. The target (ground truth) item "It's You Babe Mini Cradle, Medium" is ranked at position 19 out of 20 items in the candidate set. After using the initial prompt, the target item holds the 16th position in the candidate set. 

% 
\input{plot/prompt-task}
\input{plot/prompts-input}
%


\subsection{Prompt Optimization (PromptOpt)}

Given the initial prompts, PromptOpt strives to refine, augment, and optimize the task description prompt with self-reflection. The detailed process is elaborated as follows.

\medskip\noindent\textbf{Collecting Error Cases}. 
We randomly sample a batch ($N_t$) of sessions from training sessions ($N$) and guide ChatGPT to generate next item predictions with the initial prompts.
Afterward, we assess the recommendation outcomes, considering sessions where the target item ranks in the bottom half of the reranked candidate set as error cases. 
The example mentioned in Section~\ref{sec:prompt-initialization} is an error case, since the ranking position of the target item by using the initial prompt is 16 out of 20 candidates. 
These error cases, indicating that the corresponding prompts are not effectively guiding LLMs in executing the recommendation task, will be utilized to further refine the prompts. We use $N_e$ ($0\leq N_e \leq N_t$) to denote the total number of such error cases. 

\medskip\noindent\textbf{Inferring Reasons}. Understanding the reasons behind these collected error cases would greatly aid in refining the prompts, consequently enhancing recommendation performance. Thus, we leverage the self-reflection ability of ChatGPT, that is, asking ChatGPT to reconsider and offer justifications rooted in the identified errors. Inspired by~\cite{pryzant2023automatic}, we adopt Prompt 3 shown below to generate $N_r$ reasons for each of the $N_e$ error cases, where the `\textit{error\_case}' includes the user session and candidate item set. 
%
\input{plot/prompt-reason}

Below are the generated reasons for one error case. 
%
\begin{itemize}[leftmargin=*]
\item \textit{One reason why the prompt could have gotten these examples wrong is that it assumes that the user's interactive intent can be accurately inferred based solely on the items within each combination. However, the prompt does not provide any information about the user's preferences, tastes, or previous interactions. Without this context, it is difficult to accurately infer the user's intent from the items alone.}
\item \textit{Another reason is that the prompt does not specify how the combinations of items within the session should be discovered. It assumes that the combinations are already known and provided as input. However, in real-world scenarios, discovering meaningful combinations of items from a user's session interactions can be a complex task. The prompt does not provide any guidance on how to perform this discovery process, which can lead to incorrect results. }   
\end{itemize}

\medskip\noindent\textbf{Refining Prompts}. With the inferred $N_r$ reasons for each error case, we now ask ChatGPT to further improve the current prompt accordingly. The prompt is illustrated below. 
%
\input{plot/prompt-refine}
%
Prompt 5 is an example of the refined prompt.
By comparing the initial task description Prompt 1 and the refined Prompt 5, we can easily note that the initial prompt is improved by considering two aspects: (1) user preference and taste and (2) the definition of item combinations. These two aspects are exactly consistent with the inferred reasons by ChatGPT. 

\medskip\noindent\textbf{Augmenting Prompts}. With the refined prompts, we further ask ChatGPT to augment prompts (Prompt 7 is an example of augmentation) with the same semantic meanings using Prompt 6. Accordingly, for the $N_e$ error cases, we finally obtain $2N_e$ prompts through refinement and augmentation. These prompts will be further selected for an iterative optimization based on their recommendation performance, as introduced in what follows. 

\input{plot/out-improve}
%
\input{plot/prompt-augment}
%

%
\input{plot/out-augment}
%
  

\input{plot/ucb}

\medskip\noindent\textbf{Evaluating Prompts}.
From the pool of $2N_e$ prompts, identifying the most efficient one based on their performance is crucial for selecting the final optimal prompt. The ideal way is to evaluate their performance with all historical user sessions. However, this method may be quite computationally expensive. To address this issue, we employ the upper confidence bound (UCB) Bandits~\cite{pryzant2023automatic} to efficiently estimate the performance. In particular, it iteratively samples one prompt based on its estimated performance and then evaluates the prompts on a random batch of training sessions ($N_v$), and finally updates its performance based on the observed performance. The process is depicted by Algorithm~\ref{alg:ucb}, where the reward is calculated by the NDCG measuring the ranking position of the target item; and $\gamma$ is the exploration parameter. With UCB Bandits, we can quickly obtain the estimated performance of the $2N_e$ prompts.

\input{plot/beam-search}

\medskip\noindent\textbf{Iterative Optimization}. 
On the basis of UCB Bandits, we then %employ the beam search to 
iteratively optimize the prompts~\cite{pryzant2023automatic}. According to the estimated performance $R$, we select the Top-$N_o$ prompts and carry these promising prompts forward to the subsequent iteration. Specifically, we first use these prompts to update the prompts in the previous iteration, and then conduct the series of tasks, including collecting error cases, inferring reasons, refining, augmenting, and evaluating prompts. This iterative loop fosters incremental enhancements and exploration among various promising prompt candidates, as depicted by Algorithm~\ref{alg:beam-search}. 
%
Prompt 8 below is an example of the final optimized prompt with the best estimated performance. Using this optimized prompt for the example session mentioned in Section~\ref{sec:prompt-initialization}, the target item has been reranked to the 11th position, advancing eight positions from its previous placement in the candidate set.    

\input{plot/out-optimal}

\subsection{Prompt Curation (PromptCura)}
With the iterative optimization, we now have the Top-$N_o$ prompts. Accordingly, one straightforward way is to choose the Top-1 prompt as the final selection due to its superior overall performance. However, we notice that although a majority of sessions achieve their peak accuracy with the Top-1 prompt, a subset of them displays the best performance with other Top prompts. This can be verified by Figure~\ref{fig:same-domain-prompt}, which shows the performance gap between the Top-1 and Top-2 prompts on the validation sessions across three real-world datasets in the domains of movie, games, and e-commerce (with bundled products)\footnote{The details of the datasets utilized in our study are introduced in Section 4.1.1.}. 
From the results, it's evident that there are data points positioned where the gap is less than zero, signifying that the Top-2 prompt surpasses the Top-1 prompt in some cases. 
%
Thus, one can come up with potential solutions: (1) ensemble the two prompts to get the compensation results; and (2) train a classifier to select the best prompt for each session. 
Nevertheless, we empirically discovered that (1) fails to yield promising results because the enhancements in the subset do not offset the declines in the majority; while (2) heavily relies on the accuracy of the classifier, thus bringing in extra uncertainty to the final performance. 

\input{plot/same-domain-validation}

Fortunately, the superior generalizability of LLMs inspires us to explore the cross-domain performance of these optimized prompts. Specifically, Figure~\ref{fig:cross-domain-validation} depicts the performance of the Top-1 prompts from the three domains on the three datasets, for instance, `Opt-Games' (in purple) refers to the Top-1 prompt in the games domain. Based on the Figure, we can easily notice that the Opt-Games consistently achieves the best performance across the three domains. One potential explanation could be attributed to the Games dataset having the shortest average session length (refer to the 'Avg. Session Length' in Table~\ref{tab:statistics}) alongside a moderate level of sparsity (as seen in 'Avg. Item Repeat Frequency' in Table~\ref{tab:statistics}). These factors collectively alleviate the challenge of identifying the optimal prompt to capture crucial information, thereby enhancing SR performance.
%
Accordingly, we select the Opt-Games as the final prompt for all domains, the efficacy of which is verified in Section 4.2.  

\input{plot/cross-domain-validation}

%\begin{itemize}
    %\item Prompt\_apo
    %\item Prompt ensemble
    %\begin{itemize}
        %\item Top-k prompt with the highest rewards
        %\item Or may cluster sessions with their optimal prompts, i.e., different groups of sessions with different patterns may have their own optimal prompts, instead of a global one
    %\end{itemize}
    %\item Prompt Sampling via the Mixture Gaussian Model
    %\item Add algorithms
%\end{itemize}



==> section/related-v0.tex <==
\section{Related Work} 
This section first provides an overview of the development of session-based recommendation (SR). Then, intent-aware SR is introduced, followed by the large language model (LLM) based SR. 

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{image/framework.pdf}
    \vspace{-0.1in}
    \caption{The overall architecture of our proposed PO4ISR paradigm.}
    \label{fig:framework}
    \vspace{-0.1in}
\end{figure*}

\subsection{Session-based Recommendation}
Early works employ \textit{conventional methods} for SR, such as frequent sequential patterns~\cite{ayres2002sequential,yap2012effective}, item- and session-level similarity (e.g., SKNN~\cite{ludewig2018evaluation,jannach2017recurrent}), Markov chain (e.g., FPMC~\cite{rendle2010factorizing}) and random walk~\cite{choi2022s}.
Later, \textit{recurrent neural networks} (RNN) have been applied to handle longer sequences assuming that adjacent items in each session are sequentially dependent. 
Specifically, GRU4Rec~\cite{hidasi2016session} is the representative model, which has been further extended for improved performance using, e.g., data augmentation~\cite{tan2016improved,wang2022generative}, new losses~\cite{hidasi2018recurrent}, parallel architecture with item features~\cite{hidasi2016parallel}, 
and cross-session information transfer~\cite{quadrana2017personalizing}.
Subsequently, the \textit{attention mechanism} has been introduced in SR to relax this assumption by emphasizing more informative items in sessions~\cite{song2023counterfactual}, such as NARM~\cite{li2017neural} and STAMP~\cite{liu2018stamp}\footnote{Our study focuses on session-based recommendation. Therefore, some popular sequential-based recommendation approaches, e.g., Bert4Rec~\cite{sun2019bert4rec} and SASRec~\cite{kang2018self} are out of our scope. Please refer to~\cite{yin2023understanding} for the detailed difference between session- and sequential-based recommendation.}.
% 
To better model the high-order transition among items, \textit{graph neural network} (GNN) based methods have been recently designed to generate more accurate item embeddings from the session graph, such as SR-GNN~\cite{wu2019session}, FGNN~\cite{qiu2019rethinking}, GC-SAN~\cite{xu2019graph}, GSL4Rec~\cite{wei2022gsl4rec}, 
GNG-ODE~\cite{guo2022evolutionary}, 
KMVG~\cite{chen2023knowledge},
and ADRL~\cite{chen2023attribute}.
Besides, many studies propose to 
better leverage both the intra- and inter-session information, e.g., GCE-GNN~\cite{wang2020global}, HG-GNN~\cite{pang2022heterogeneous}, 
DGNN~\cite{guo2022learning},
SPARE~\cite{peintner2023spare}, CGSR~\cite{yu2023causality}, 
and HADCG~\cite{su2023enhancing}.
%
%Meanwhile, GSL4Rec~\cite{wei2022gsl4rec} learns graph structure from social neighbors for better user interest inference.
%
%GNG-ODE~\cite{guo2022evolutionary} learns dynamic user preference by modeling a session as a continuous-time temporal session graph. 
%
%CGSR~\cite{yu2023causality} effectively blocks the impact of the shortcut path on the session graph from a casual perspective.
%
Meanwhile, other works (e.g., $S^2$-DHCN~\cite{xia2021self} and CoHHN~\cite{zhang2022price}) employ hypergraphs to enhance item representations for SR. 




\subsection{Intent-aware Session Recommendation}
An essential line of research learns the intents hidden in the session for more accurate SR. 
Early studies assume items inside a session are associated with one (implicit) purpose. In particular, NARM~\cite{li2017neural} extracts the last hidden state as the session representation and applies an attention mechanism on all hidden states to learn the user’s intention. 
%
STAMP~\cite{liu2018stamp} explicitly emphasizes the current interest reflected by the last click to capture the hybrid features of current and general interests from previous clicks via an attention network. 
%
SR-GNN~\cite{wu2019session}, GC-SAN~\cite{xu2019graph}, and GCE-GNN~\cite{wang2020global} model each session as graph-structured data and
apply GNN to learn the representations of user intents with attention networks.
%
TAGNN~\cite{yu2020tagnn} 
%equips a target attention module to 
adaptively activates user intents by considering the relevance of historical behaviors given a target item. 
%
LESSR~\cite{chen2020handling} 
learns better local and global interests as the user's intent representation by easing the information loss issues.
%
MSGAT~\cite{qiao2023bi} utilizes similar sessions to efficiently generate the session intent representation.
%
Nonetheless, a session may encompass items with varying intentions. Thus, solely modeling the main intention could lead to information loss, potentially hurting the performance of SR.

Therefore, recent studies endeavor to learn multiple intentions hidden in a session for more effective SR. Specifically, 
%
NirGNN~\cite{jin2023dual} learns the dual intents from the angle of an attention mechanism and data distribution in the session graph. 
%
MCPRN~\cite{wang2019modeling} designs mixture-channel purpose routing networks to detect the purposes of each item inside a session and assign them to the corresponding channels. 
%
IDSR~\cite{chen2020improving} projects the item representation into multiple spaces indicating various intentions and employs self-attention within each space to capture distinct intentions.
%
HIDE~\cite{li2022enhancing} splits an item embedding into multiple chunks to represent different intentions and then organizes items in a session with hyperedges to facilitate the learning of associated intentions.  
%
MIHSG~\cite{guo2022learning} and Atten-Mixer~\cite{zhang2023efficiently} learn multi-granularity consecutive user intent units to generate more accurate session representations.
%
DAGNN~\cite{yang2022dagnn} extracts the session demands over the whole item category space to capture semantically correlated categories for better SR.
%
STAGE~\cite{li2022spatiotemporal} captures the impact of both spatiotemporal context and multiple intrinsic intents in a session. 
%
ISCON~\cite{oh2022implicit} generates implicit session intents as novel features to enhance next-item prediction.
%

Despite the success, these methods suffer from two major limitations: (1) they make the impractical assumption that all sessions have a uniform and fixed number of intentions, either single or multiple ones; and (2) they can only learn intentions in the latent space, restricting the transparency of the SR. In contrast, our method seeks to learn a dynamic number of semantic intents hidden in a session for more accurate and explainable SR, using the advanced logical reasoning ability of LLMs.    



\subsection{LLM-based Session Recommendation}
LLMs have achieved remarkable achievements for effective recommendation~\cite{dai2023uncovering,he2023large,sanner2023large,bao2023tallrec}. However, only a few are designed for SR, for instance, NIR~\cite{wang2023zero} adopts zero-shot prompting for the next-movie recommendation.
%
%sequential rec
Most methods target sequential recommendation. Among them, some leverage the in-context learning (ICL) capability of LLMs. For instance, 
\citeauthor{harte2023leveraging}~\cite{harte2023leveraging} exploit the power of LLMs by, e.g., using embeddings obtained from LLMs to initialize Bert4Rec~\cite{sun2019bert4rec}.
%
\citeauthor{hou2023large}~\cite{hou2023large} use LLMs as rankers by designing sequential, recency-focused, and ICL prompting.
%
Others align LLMs for recommendation via fine-tuning. To be specific,
BIGRec~\cite{bao2023bi} employ LLMs
%explores the capability of LLMs 
in an all-rank scenario by grounding LLMs to the recommendation and actual item spaces.
% 
TransRec~\cite{lin2023multi} identifies fundamental steps of LLM-based recommendation 
%(i.e., item indexing and generation grounding) 
to bridge the item and language spaces.
%
%Similarly, GenRec~\cite{ji2023genrec} uses the understanding ability of LLMs to directly generate the target item to recommend. 
%
GPT4Rec~\cite{li2023gpt4rec} generates multiple queries given item titles in a user's history with beam search and then retrieves items for recommendation by searching these queries with a search engine. 
%
LlamaRec~\cite{yue2023llamaRec} uses an ID-based sequential recommender as the retriever to generate candidates and then designs a verbalizer to transform LLM output as the probability distribution for ranking. 
%
Moreover,
RecInterpreter~\cite{yang2023large} examines the capacity of LLMs to decipher the representation space of sequential recommenders with sequence-recovery and -residual tasks.

However, the potential of LLMs cannot be harnessed solely through simple ICL (e.g.,~\cite{wang2023zero}). While fine-tuning LLMs for recommendation shows promising results, it is constrained by the computational demands and availability of open-source LLMs. Instead, we propose a new paradigm for ISR by automatically optimizing prompts, which efficiently prompts LLMs to semantically comprehend the session-level user intents, thus promoting the delivery of more accurate and understandable SR.   




==> section/related.tex <==
\section{Related Work}
This section presents a detailed literature review on session-based recommendation (SR). In particular, we first provide an overview of the technique development of SR. Then, we introduce intent-aware session recommendation, followed by the large language model (LLM) based session recommendation. 

\subsection{Session-based Recommendation}
Early works mainly adopt \textit{conventional methods } for SR. For instance, some approaches are based on the identification of frequent sequential patterns for next item recommendation~\cite{ayres2002sequential,yap2012effective}. Session-based KNN (SKNN)~\cite{ludewig2018evaluation,jannach2017recurrent} considers both item- and session-level similarity. FPMC~\cite{rendle2010factorizing} combines matrix factorization (MF)~\cite{koren2009matrix} with Markov Chain (MC) to better deal with sequential relationship between items.  
Later, \textit{recurrent neural networks} have been applied using longer sequence for better prediction. For instance, GRU4Rec~\cite{hidasi2016session} is the first to apply recurrent neural network to capture the long-term dependency in a session. It has been further extended for improved performance, such as, adopting data augmentation~\cite{tan2016improved}, new losses~\cite{hidasi2018recurrent}, parallel architecture with item features~\cite{hidasi2016parallel} and cross-session information transfer~\cite{quadrana2017personalizing}.
Subsequently, the \textit{attention mechanism} has been introduced in SR\footnote{Our study focuses on session-based recommendation. Therefore, some popular sequential-based recommendation approaches, e.g., Bert4Rec~\cite{sun2019bert4rec} and SASRec~\cite{kang2018self} are out of our scope. Please refer to~\cite{yin2023understanding} for the detailed difference between session- and sequential-based recommendation.}. For instance, NARM~\cite{li2017neural} explores a hybrid encoder with an attention mechanism to capture the item-transition information among items in every session. STAMP~\cite{liu2018stamp} uses simple MLP networks and an attentive network to capture both users’ general and current interests. 

However, the above methods always model single-way transitions between consecutive items and neglect the transitions among other items in the session. Hence, \textit{graph neural network (GNN) based methods} have been designed in recent years. For instance, SR-GNN~\cite{wu2019session} imports GNNs to generate more accurate item embedding vectors from the session graph. FGNN~\cite{qiu2019rethinking} adopts a weighted graph attention network to enhance SR-GNN, whilst GC-SAN~\cite{xu2019graph} replaces the simple attention network with self-attention to capture long-range dependencies. 
LESSR~\cite{chen2020handling} resolves the lossy session encoding and ineffective long-range dependency capturing problems for better SR.
TAGNN~\cite{yu2020tagnn} uses target-aware attention such that the learned session representations vary with different target items. 
Furthermore, GCE-GNN~\cite{wang2020global} learns session representations over both the current session graph and all-session graph. 



\subsection{Intent-aware Session Recommendation}
An essential line of research models the intents hidden in the session for more accurate SR. Early works assume items inside a session are associated with one (implicit) purpose. In particular, NARM~\cite{li2017neural} extracts the last hidden state as the session representation and applies an attention mechanism on all hidden states to learn the user’s intention. 
%
STAMP~\cite{liu2018stamp} explicitly emphasizes the current interest reflected by the last click to capture the hybrid features of current and general interests from previous clicks via the attention network. 
%
SR-GNN~\cite{wu2019session} models each session as graph-structured data and represents it as the composition of the global interest and the current interest of that session using an attention network.
LESSR~\cite{chen2020handling} 
learns better local and global interest as the session representation by easing the information loss issues in GNN-based SR.
%
TAGNN~\cite{yu2020tagnn} equips a novel target attention module to adaptively activate user interests by considering the relevance of historical behaviors given a target item. 
%
Nonetheless, a session may encompass items with varying intentions. Thus, solely modeling the main intention could lead to information loss, potentially hurting the performance of SR.

Hence, recent studies endeavor to learn multiple intentions hidden in a session for more effective SR. Specifically, MCPRN~\cite{wang2019modeling} designs mixture-channel purpose routing networks to detect the purposes of each item inside a session and assign them to the corresponding channels. 
%
IDSR~\cite{chen2020improving} projects the item representation into multiple spaces, where each space corresponds to a specific intention. It then employs the self-attention mechanism within each space to capture distinct intentions.
%
HIDE~\cite{li2022enhancing} split the item embedding into multiple chunks, each corresponding to an intention. By organizing items within a session using hyperedges, it facilitates the learning of intentions associated with those items. Despite their effectiveness, these methods suffer from two major limitations: (1) they assume all sessions have the same number of intentions, which is impractical; and (2) they can only learn the latent intentions, severely restricting the transparency of the SR.  

%\begin{itemize}
    %\item Implicit intent-based methods
    %\begin{itemize}
        %\item Single intent-based methods
        %\item Multiple intent-based methods
    %\end{itemize}
    %\item Explicit intent-based methods
    % \begin{itemize}
    %     \item The one use category to represent different intents
    %     \item need to search more related works
    % \end{itemize}
%\end{itemize}

\subsection{LLM-based Session Recommendation}


